ConceptHash: Interpretable Fine-Grained Hashing via Concept Discovery

Existing fine-grained hashing methods typically lack code interpretability as they compute hash code bits holistically using both global and local features. To address this limitation, we propose ConceptHash, a novel method that achieves sub-code level interpretability. In ConceptHash, each sub-code corresponds to a human-understandable concept, such as an object part, and these concepts are automatically discovered without human annotations. Specifically, we leverage a Vision Transformer architecture and introduce concept tokens as visual prompts, along with image patch tokens as model inputs. Each concept is then mapped to a specific sub-code at the model output, providing natural sub-code interpretability. To capture subtle visual differences among highly similar sub-categories (e.g., bird species), we incorporate language guidance to ensure that the learned hash codes are distinguishable within fine-grained object classes while maintaining semantic alignment. This approach allows us to develop hash codes that exhibit similarity within families of species while remaining distinct from species in other families. Extensive experiments on four fine-grained image retrieval benchmarks demonstrate that ConceptHash outperforms previous methods by a significant margin, offering unique sub-code interpretability as an additional benefit. Code at: https://github.com/kamwoh/concepthash.

==> texs/correlation_impact.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[keepaspectratio, width=\linewidth]{figs/correlation_context.pdf}
        \caption{Without $\mathcal{L}_\text{decorr}$}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[keepaspectratio, width=\linewidth]{figs/correlation_context_mincs.pdf}
        \caption{With $\mathcal{L}_\text{decorr}$}
    \end{subfigure}
    \caption{Impact of $\mathcal{L}_\text{decorr}$ on the correlation matrix between the $M=8$ visual context tokens $[V]$ from 1st layer to 12th (last) layer of the visual encoder. Brighter color indicates higher cosine similarity and darker color indicates lower cosine similarity, the value on top is the maximum cosine similarity between the context tokens.}
    \label{fig:correlation}
\end{figure}


==> texs/fg_map_noadapter.tex <==
%%%% 4 datasets %%%%%
\begin{table*}[t]
    \caption{Performance of different methods for 3 different bits on different benchmark datasets. \textbf{Bold} values indicate the best performance in the column. Note that ITQ is an unsupervised hashing method that projects embeddings into hash codes, hence we can see it as the baseline performance. \todo{note: frozen}}
    \centering
    \adjustbox{max width=\textwidth}{
        \begin{tabular}{l|ccc|ccc|ccc|ccc}
        \toprule
            Datasets & \multicolumn{3}{c|}{CUB-200-2011} & \multicolumn{3}{c|}{NABirds} & \multicolumn{3}{c|}{Aircraft} & 
              \multicolumn{3}{c}{CARS196}  \\
              \midrule
            Methods & 16 & 32 & 64 & 16 & 32 & 64 & 16 & 32 & 64 & 16 & 32 & 64 \\
            \midrule
            ITQ \cite{itq2012gong} & 7.82 & 11.53 & 15.42 & 3.40 & 5.50 & 7.60 & 8.12 & 9.78 & 10.87 & 7.80 & 11.41 & 15.16 \\
            \midrule
            HashNet \cite{hashnet2017cao} & 12.28 & 16.02 & 18.35 & 5.05 & 6.81 & 7.84 & 10.51 & 12.39 & 14.59 & 12.63 & 16.98 & 20.30 \\
            DTSH \cite{dtsh2016wang} & 19.42 & 22.29 & 24.78 & 6.71 & 8.24 & 10.62 & 13.49 & 16.28 & 16.82 & 18.51 & 22.38 & 27.54 \\
            GreedyHash \cite{greedyhash2018su} & 14.50 & 29.25 & 37.78 & 4.50 & 14.01 & 19.76 & 16.09 & 20.63 & 22.84 & 17.35 & 31.69 & 37.80 \\
            CSQ \cite{csq2020yuan} & 6.63 & 14.93 & 26.90 & 2.12 & 4.93 & 10.19 & 11.68 & 17.79 & 24.67 & 7.89 & 16.36 & 27.13 \\
            DPN \cite{dpn2020fan} & 7.47 & 16.42 & 27.26 & 2.55 & 5.65 & 10.61 & 12.09 & 18.44 & 23.69 & 9.04 & 17.79 & 28.94 \\
            OrthoHash \cite{ortho2021jk} & 6.83 & 14.74 & 24.87 & 2.45 & 5.12 & 10.74 & 11.24 & 17.30 & 23.61 & 7.88 & 15.99 & 27.52 \\
            \midrule
            CSQ + LG \cite{csq2020yuan} & 19.24 & 26.10 & 31.52 & 8.83 & 12.90 & 15.85 & 17.90 & 21.14 & 24.54 & 22.01 & 29.17 & 34.17 \\
            DPN + LG \cite{dpn2020fan} & 20.12 & 27.11 & 32.32 & 9.30 & 13.43 & 16.44 & 18.27 & 21.53 & 24.74 & 22.74 & 29.88 & 35.14 \\
            OrthoHash + LG \cite{ortho2021jk} & 18.51 & 25.67 & 31.59 & 8.83 & 12.92 & 15.89 & 16.00 & 20.54 & 25.43 & 21.47 & 29.20 & 35.09 \\
            \midrule
            A$^2$-Net \cite{wei2022a2net} & 20.87 & 35.18 & 42.59 & 7.29 & 12.77 & 19.27 & 22.27 & 31.56 & 30.72 & 20.09 & 33.90 & 45.42 \\
            SEMICON \cite{shen2022semicon} & 39.10 & 43.46 & 43.53 & 22.59 & 24.50 & 25.03 & 31.72 & 33.08 & 32.11 & 47.81 & 51.12 & 50.83 \\
            \midrule
            ConceptHash-8 (Ours) & 48.02 & 49.08 & 45.59 & 23.34 & 30.36 & 29.33 & 34.95 & 35.68 & 37.80 & 51.39 & 55.22 & 43.49 \\
            ConceptHash-16 (Ours) & \bf 51.65 & \bf 52.18 & \bf 57.75 & \bf 28.33 & \bf 28.51 & \bf 37.01 & \bf 40.21 & \bf 40.48 & \bf 39.25 & \bf 56.70 & \bf 60.67 & \bf 63.72 \\
             \bottomrule 
        \end{tabular}
    }
    \label{tab:fg_mAP}
\end{table*}

==> texs/pr.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{\textwidth}
        % \includegraphics[draft, width=0.33\linewidth, height=100pt]{figs/foo.pdf}
        \centering
        \includegraphics[keepaspectratio, width=\linewidth]{figs/pr_legend.pdf}
        \includegraphics[keepaspectratio, scale=0.455]{figs/p@h_cub200.pdf}
        \includegraphics[keepaspectratio, scale=0.455]{figs/pr_cub200.pdf}
        \includegraphics[keepaspectratio, scale=0.455]{figs/p_cub200.pdf}
        \caption{CUB-200-2011}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \includegraphics[keepaspectratio, scale=0.455]{figs/p@h_cars196.pdf}
        \includegraphics[keepaspectratio, scale=0.455]{figs/pr_cars196.pdf}
        \includegraphics[keepaspectratio, scale=0.455]{figs/p_cars196.pdf}
        \caption{CARS196}
    \end{subfigure}
    \caption{(Left to Right): Precision within different hamming radius, precision-recall curve, and precision curve w.r.t. top-$R$. 16-bit hash codes are used for both (a) CUB-200-2011 and (b) CARS196. }
    \label{fig:pr}
\end{figure*}

